Viko: An Adaptive Gecko Gripper with Vision-based Tactile Sensor

Monitoring the state of contact is essential for robotic devices, especially grippers that implement gecko-inspired adhesives where intimate contact is crucial for a firm attachment. However, due to the lack of deformable sensors, few have demonstrated tactile sensing for gecko grippers. We present Viko, an adaptive gecko gripper that utilizes vision-based tactile sensors to monitor contact state. The sensor provides high-resolution real-time measurements of contact area and shear force. Moreover, the sensor is adaptive, low-cost, and compact. We integrated gecko-inspired adhesives into the sensor surface without impeding its adaptiveness and performance. Using a robotic arm, we evaluate the performance of the gripper by a series of grasping test. The gripper has a maximum payload of 8N even at a low fingertip pitch angle of 30 degrees. We also showcase the gripper's ability to adjust fingertip pose for better contact using sensor feedback. Further, everyday object picking is presented as a demonstration of the gripper's adaptiveness.

==> 2rela.tex <==
\section{Related Works}

Human use re-grasp, pose transition and deformable adaptation on fingertip for the dexterity of grasping and manipulations targeting to distinct objects in the daily activities. Inspired from the bio-archetype, a number of studies are focusing on building an artificial hand that can mimic its skills. On one hand, employing re-grasp and pose transition for in-hand manipulation strategies has been widely studied from various aspects, showing great potentials in applications \cite{ma2011dexterity,antonova2017reinforcement,chavan2020planar}. On the other hand, the fingertip adaptation is still mainly developed and utilized for applications in the state of passive morphing via self-deformation of the soft material \cite{crooks2016fin,song2018fingertip,chavan2015two} or the flow characteristic of fluidic media \cite{brown2010universal,hou2019design}. Thus, while the passive morphing fingertip allows for limited dexterous in-hand manipulation \cite{hang2016hierarchical,sundaralingam2017relaxed}, an active morphing strategy is required for dexterous manipulations with more flexibility.

\subsection{Variable-frictional fingertip}

For the variety of properties on the fingertip, several researchers made efforts on the frictional change on the contact surface to alter the grasping performance. Becker et al. have proposed a friction switch mechanism for robotic hands via a pneumatic actuator \cite{becker2017tunable} The adhesive-inflatable surface beneath the slippery plane can be extracted through holes installed on the slippery surface. The presented design is an extendedly active morphing strategy to the passive counterpart made by Spiers et al. \cite{spiers2018variable} which could switch to high-friction mode through force exerted in the finger. Other than friction variations on the solid pads, Mizushima et al. \cite{mizushima2019deformable} utilized lubricant to reduce friction coefficient for varying the contact environment. In addition, origami structure is also discovered for its morphing capability on the friction variation by shifting the inserted high friction surfaces using cable tension \cite{lu2020origami}.

\subsection{Cavity-shaped morphing fingertip for pivoting}

For processing fine manipulations and re-grasping tasks, multiple simple-structured two-phase hands rising extrinsic or intrinsic resources have been reported \cite{chavan2015two,chavan2018pneumatic,he2020soft}. They use mainly similar V-groove cavity structure on the parallel gripper to passively or actively reorient prismatic objects from a horizontal pose to an upright secured pose. When switching to upright secure mode, the soft materials employed, e.g. strip and silicon covering, will recede into the cavity, wrapping the cylinder and allowing contacts with the cavity. Thus an easy transition method between a firm grasp and a pinch grasp for free pivoting can be generated.

% \subsection{Passive morphing fingertip with fluid media}

% A vacuum-sealed package of granular beans is solid, yet becoming soft and flexible as relaxed. The granular jamming mechanism underlying can determine the morphology of the entire structure. From the bulky gripper \cite{brown2010universal} to the tiny fingertip \cite{hou2019design}, the morphing structures can adapt to target objects with a large range of dimensions. The adaptability depends on the bean size and the smoothness of the bean surface which affects the fluidic movement. However, the morphing strategy passively depends on the contact fit with the target.

In addition, Song et al. \cite{song2018fingertip} also put forward a collection of manipulation primitives for the representatives of contact features and three designed fingertips are evaluated for the effectiveness for a firm grasping facing different local surfaces. However, these primitives are manually fixed, which is lack of automation and not considerate for product transition of assembly line. Therefore, in order to extend the availability of the fingertip primitives, an active morphing strategy is proposed in this work with multiple morphing configurations for dexterous manipulations.


==> acknowledgment.tex <==
\section*{Acknowledgment}
Here we would like to thank Lei Tai for his insight into our framework.
